Unlabelled landmark matching via Bayesian data selection, and application to cell matching across imaging modalities

We consider the problem of landmark matching between two unlabelled point sets, in particular where the number of points in each cloud may differ, and where points in each cloud may not have a corresponding match. We invoke a Bayesian framework to identify the transformation of coordinates that maps one cloud to the other, alongside correspondence of the points. This problem necessitates a novel methodology for Bayesian data selection; simultaneous inference of model parameters, and selection of the data which leads to the best fit of the model to the majority of the data. We apply this to a problem in developmental biology where the landmarks correspond to segmented cell centres, where potential death or division of cells can lead to discrepancies between the point-sets from each image. We validate the efficacy of our approach using in silico tests and a microinjected fluorescent marker experiment. Subsequently we apply our approach to the matching of cells between real time imaging and immunostaining experiments, facilitating the combination of single-cell data between imaging modalities. Furthermore our approach to Bayesian data selection is broadly applicable across data science, and has the potential to change the way we think about fitting models to data.

==> extra_stuff.tex <==
%intro stuff 

%The probability distribution of potential models and respective parameters (hypotheses) is known as the posterior distribution and the solution with the highest probability in the posterior known as the maximum a posteriori, or MAP, estimate. The posterior distribution is given by Bayes' theorem through the combination of observations and an associated likelihood, along with prior knowledge on the model parameters. The major appeal of a Bayesian approach to an inverse problem is the description of the relative uncertainty in any identified solution.

%Markov Chain Monte Carlo (MCMC) techniques are routinely used to facilitate exploration of complex posterior distributions of inverse problems \cite{gelman2003,Risholm2013}. MCMC methods like the random walk Metropolis Hastings algorithm \cite{hastings1970monte}, sample on model parameters by constructing an ergodic Markov chain whose stationary distribution agrees with the posterior distribution of interest. After some period of sampling, in part determined by the complexity of the model and problem, the distribution of accepted parameters allows for the identification of the MAP estimate along with quantification uncertainty in the model parameters that have been sampled on.



%The preimplantation period is the time between fertilisation of the egg by the sperm and the time of implantation into the uterus wall. It is a crucial period within development where three cell lineages are specified and organised. If the cell lineages do not specify and organise themselves correctly, the pregnancy will ultimately fail \cite{plusa2020, Taft2008}.  The trophectoderm (TE), primitive endoderm (PrE) and epiblast (Epi) are formed during the preimplantation period and go on to form extra-embryonic lineages and the embryo proper \cite{plusa2020}. Towards the end of the preimplantation period the embryo resembles a robust, three dimensional morphology with a shell of TE cells, a population of Epi cells at one pole of the embryo (inside of the TE), and a layer of PrE cells between the Epi population and a fluid-filled cavity at the opposing embryo pole. How the Epi and PrE lineages specify from a homogeneous population of cells is still not fully understood, but it appears to involve molecular and architectural control of the embryo as well as cell developmental history \cite{fischer2020, Forsyth2021}. 

%Imaging modalities within developmental biology have pushed forward our understanding of embryo development, providing insights into the dynamics of molecular and cellular control within relevant biological processes . The evolution of microscopic techniques has allowed for better imaging of three dimensional structures, visualisation of proteins and characterisation of temporal features within development \cite{Iyer2021,Weniger2004}. For example, real time imaging (RTI) techniques which involve the culture and three dimensional imaging of live embryos over a period of development allows for characterisation of overall embryo architecture \cite{Abe2013, grabarek2012}. By combining RTI with mouse reporter lines, such as the H2b:GFP strain, spatio-temporal information at the single cell level can additionally be extracted through the tracking of fluorescent cell nuclei \cite{Hadjantonakis2004}. In addition to the more sophisticated RTI experiments, there are widely used classical immunohistochemistry (immunostaining) approaches that are performed on fixed embryos (no longer developing) \cite{Abe2013,plusa2008}. Immunostaining involves the specific targetting of proteins using antibodies and secondary attachments of fluorophores to enable visualisation of protein abundance. This technique has been used extensively to interrogate the influence of protein expression on cell fate and embryo development, however it is limited by the lack of historical cell information, believed to be a key factor in early cell specification events in the mammalian preimplantation period \cite{Morris2010,Yamanaka2010}. 
 
%In order to understand the specification of the Epi and PrE, we need to be able to understand the influence of spatio-temporal cues on protein expression and vice versa \cite{ryan2019,fischer2020,saiz2013, Forsyth2021}. An ideal approach to gather cell history and protein expression data is to culture embryos within an RTI experiment and perform subsequent immunostaining treatments. Until now, such experiments have been performed with manual matching of cells between RTI movies and immunostaining images using markers such as dividing cells or cells undergoing apoptosis. The manual matching of cells is non-trivial in three dimensions and can sometimes lead to low accuracy data sets. We therefore present a quantitative, Bayesian approach to match cells across imaging modalities, for example RTI and immunostaining. %could cite  \cite{Simon2020} here because they do manual matching but not sure if we want to be too savage? depends? 






\subsubsection{Affine and Non-Linear Transformation}
To make proposals on $\mathbf{\varphi}$ and $\mathbf{p}$, we use an adaptive random walk approach that follows
\begin{equation}
v=u + \beta_t \xi;
\end{equation}
 with a step-size $\beta_t$ and $\xi\sim N(0,C)$. As we have included the local deformation as an optional module, $C= 12 \times 12$ or $C=(12+3n_2) \times (12+3n_2)$.The covariance matrix, $C$, is estimated by using the previous $x$ thinned samples during tempering, as to avoid biasing of $C$ due to samples obtained at temperatures significantly different to the current temperature. Whereas C is estimated using an online algorithm, at $T=1$ as to use the entire sample set without having to save all variables during sampling at $T=1$. The covariance is first updated at $x$ iterations, and then updated at $x1=1.1 x0$ iterations, where $x0$ is the previous check iteration number. the non-linear update of the covariance matrix was enforced in order satisfy the diminshing adaptivity condition. 
 
The acceptance ratio was calculated as 
\begin{equation}
\alpha=  \min \left( 1, \frac{\pi_0(\varphi_1,\mathbf{p}_1)}{\pi_0(\varphi_0,\mathbf{p}_0)} \exp \left( \frac{1}{T}(\Phi(X_0,F, \nu, \Psi, n_1) - \Phi(X_1,F, \nu, \Psi, n_1)) \right) \right)\\
\end{equation}
where $\Phi$ is the negative log of the posterior predictive described in equation \ref{eq:postpred}, $X_1= Y^1 - \mathcal{G}([\mathbf{\varphi_1}, \mathbf{p_1}, P])$ and $X_0= Y^1 - \mathcal{G}([\mathbf{\varphi_0}, \mathbf{p_0}, P])$ where the subscripts zero and one indicate the current and proposed values of $\mathbf{\varphi}$ and $\mathbf{p}$ respectively. The step-size parameter, $\beta_t$ is tuned to achieve an acceptance rate of $0.234\pm 0.1$, for optimum efficiency as discussed in \cite{gelman1997}, and checked every $f_c$ iterations to allow for adaptation of the sampling. 

To account for potential untrue matches within the datasets we include a match selection approach, which aims to describe fidelity parameters for each data point that act to temper out their contribution to the likelihood when their dynamics can not be encapsulated by out model.\\
To efficiently make proposals on $\mathbf{f}$, we define a map, $\tilde{T}(f)=\log(\frac{1}{f}-1)$ , mapping together $\tau$ and the fidelity terms. This map results in $\tau\in[-\infty,\infty]$ as $f\in[0,1]$. As the terms are bijective, and $\tau$ determined over all values, we can perform random walk proposals on $\tau$ and invert to obtain proposed values of $f$. Proposals on $\tau$ are made using 
\begin{equation}
\tau_1 = \tau_0 + \beta_\tau  \xi,
\end{equation}
for $\xi \sim \mathcal{N}(0,1)$ and the fidelity terms calculated using the inversion of the map, $\tilde{T}$, on $f$
\begin{equation}
f_1 = \frac{1}{\exp(\tau_1)+1}.
\end{equation} 
When constructing the acceptance ratio on the proposals of $f$, we must be careful to pull through the appropriate proposal density as proposals made on $\tau$ and thus $f$ are no longer symmetric. We therefore calculate the conversion of the proposal density onto $f$ by comparing the gradient of the proposal distribution through 
\begin{equation}
\frac{d\tilde{T}}{df} = \frac{1}{f(f-1)},
\end{equation}
thus allowing us to describe proposal density comparison term as 
\begin{equation}
\frac{p(f_0|f_1)}{p(f_1|f_0)}=\prod_{i=1:n} \frac{f_1^i(f_1^i-1)}{f_0^i(f_0^i-1)}.
\end{equation}
We are then able to write the acceptance ratio as 
\begin{equation}
\alpha=\min\left(1, \frac{\pi_0(\mathbf{f_1})}{\pi_0(\mathbf{f_0})} \exp\left(\frac{1}{T} (\Phi(X,F_0, \nu, \Psi, n_1) - \Phi(X,F_1, \nu, \Psi, n_1))\right) \frac{p(f_0|f_1)}{p(f_1|f_0)}\right),
\end{equation}
where $F_0$ and $F_1$ are indicative of the current and proposed fidelity matrices respectively and $X=Y^1 - \mathcal{G}([\mathbf{\varphi}, \mathbf{p}, P])$.\\ 
Standard RW proposals have been shown in to have an optimum acceptance rate, $\bar{\alpha=0.234}$, for an N-dimensional Gaussian target distribution \cite{gelman1997}, to ensure this still held for this approach of sampling indirectly on $f$, we performed sampling on the fidelity terms of an $n=8$ point test problem, where each point has an increasing level of `mismatch' or difference between 0 and 10. Points with greater mismatches are expected to have lower fidelity terms, in order to tune out their contribution to the likelihood. We performed the experiment for a series of different optimum acceptance rates between 0.15 and 0.85, with a 0.1 tolerance, for $N=1\times 10^4$ iterations. By calculating the multi estimated sample size (multiESS)\cite{Vats2019}, we were able to show an increase in mESS and mESS$//$s around the optimum acceptance rate of 0.25, therefore agreeing with the previous assumption of optimum algorithm efficiency at $\bar{\alpha}= 0.234 $. \\
\begin{figure}[h]
\begin{center}
\includegraphics[width=0.65\textwidth]{fig2}
\end{center}
\caption{Identification of optimum acceptance rate for the match selection module of the algorithm. The calculated multiESS and multiESS/s for each optimum acceptance rate ($\bar{\alpha}$)and compared to the standard optimum of 0.234 for RW proposals (dashed line). }
\label{fig:fidproof}
\end{figure}


\begin{table}[h] \label{table:fidtests}
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Stage} & \textbf{Number of Cells} & \textbf{Number of True Matches} & \textbf{Number of Untrue Matches} \\ \hline
8              & 7                        & 6                               & 1                                 \\ \hline
16             & 13                       & 11                              & 2                                 \\ \hline
32             & 30                       & 27                              & 3                                 \\ \hline
64             & 58                       & 52                              & 6                                 \\ \hline
\end{tabular}
\end{table}


\jf{\begin{itemize}
    \item key findings from the research, and link to overarching aim of research (what should readers take from this work?) : \edit{we are able to match cells between imaging modalities or more generally , we are able to match points with minimal constraints on initial conditions and obtain correct matchings and associated uncertainties}
    \item place the findings in context, go back to literature results and describe how the work fits in with the current approaches  \edit{other approaches are typically optimisation approaches, use mixture models to describe the matching of subsets of points, some dont directly sample on the midentification of transformation params and instead use procurstes algorithm} 
    \item mention and discuss any unexpected results along with potential reasons + describe why it is important to the research question \edit{ability of data selection to improve mixing of chains} 
    \item address limitations or weaknesses in the research \edit{dimensionality? }
    \item follow-ups and further research \edit{talk about the inclusion of data selection using conjugate priors?, use other information e.g. point relations}
    \item restatement of the most significant findings and why it is important in general applications
\end{itemize} 
} 


% \begin{table}[htbp]
% \centering
% \begin{tabular}{|l|l|l|l|}
% \hline
% Non-linear deformations   & Bayesian data selection       & $\textrm{min}(\tilde{d})$ & $\textrm{min}(\tilde{d_u})$ \\ \hline
% \ding{52} & \ding{55}& 0.526                                & 0.335                                  \\ \hline
% \ding{55}& \ding{55}& 1.15                                 & 0.358                                  \\ \hline
% \ding{52} & \ding{52} & 0.0943                               & 0.0829                                 \\ \hline
% \ding{55}& \ding{52} & 1.26                                 & 0.0342                                 \\ \hline

% \end{tabular}
% \caption{Summary of minimum (over the 8 chains) median cell to match distances for all cells $\tilde{d}$ and for the cells not subject to a deformation $\tilde{d_u}$. }\label{tab:defstats}
% \end{table}



%%%%deformation section 

We next sought to test the incorporation of non-linear deformations within the transformation. We generated a test problem based on the 33-cell data set where we assigned non-zero momenta (drawn from the prior) to all points where $x<0$, values given in supplementary table \ref{tab:datagenparamvalues}. In total, 18 points were assigned a non-zero momentum, and therefore deformed explicitly through equations \ref{eq:deftosolve_pos} and \ref{eq:deftosolve_mom}. The deformed points were then subject to an affine transformation, parameters given in supplementary table \ref{tab:datagenparamvalues} and subject to noise of the form $\mathcal{N}(0,0.01^2I_3)$. 

%\slc{I feel like the next two subsubsections could be unified - their results are already given in a single table and a single figure, and only differ by the inclusion of BDS. This should lead to a significant reduction in text too, which will probably be enough to get us to below 8000 words. Please have a go, and then I'll take another look.}

First we attempted to match the points by sampling on the affine parameters, the deformation momenta, and the permutation only, i.e. excluding data selection, test a). Due to the increased number of parameters (by $3n$), we increased the number of tempered iterations to $N=10^7$ iterations, thereby reducing the cooling rate. 

All 8 chains converged to different permutation vectors, with between 0 and 19 incorrect matches. The fact that there is such a high failure rate with such a slow cooling rate suggests a very rough and difficult energy landscape to sample from in this problem. The chain with zero errors in the permutation vector, showed good spatial matching of points using the MAP estimators of the transformation. We identified that this chain had the minimum negative log of the posterior post-optimisation and so for all future comparisons of the cell to match distance we present the corresponding distances from the chain with the minimum negative log posterior after optimisation. The median cell to match distance, $\tilde{d}$ was equal to 0.526 units, table \ref{tab:defstats}. The cells not assigned a momentum during initial generation of the test problem, had a median cell to match distance, $\tilde{d_u}$ equal to 0.335. 

\edit{ \begin{table}[htbp]
\centering
\begin{tabular}{|l|l|l|}
\hline
Test       & $\textrm{min}(\tilde{d})$ & $\textrm{min}(\tilde{d_u})$ \\ \hline
a & 0.526                                & 0.335                                  \\ \hline
b & 1.15                                 & 0.358                                  \\ \hline
c & 0.0943                               & 0.0829                                 \\ \hline
d & 1.26                                 & 0.0342                                 \\ \hline

\end{tabular}
\caption{Summary of median cell to match distances for all cells $\tilde{d}$ and for the cells not subject to a deformation $\tilde{d_u}$. Values given corresponding to the chain with the lowest negative log of the posterior post optimisation.}\label{tab:defstats}
\end{table}} 

We also tested this problem without sampling on the momenta for the deformation, test b) (i.e. just sampling on the affine transformation and permutation vector). %This test serves as a comparison when we know some of the data cannot be matched through the model that does not incorporate non-linear deformation. 
The number of tempered iterations was reduced to $N=7\times 10^6$ as we were no longer sampling on the $3n$ momentum parameters. Interestingly, 4/8 chains converged to the correct permutation vector, and the remaining chains only had 4 incorrect matches. However, $\tilde{d}$ was significantly increased to a value of 1.15 units, table \ref{tab:defstats}, indicative of an overall worse matching of points and reduced performance without the explicit inclusion of the non-linear deformation. 

%We then wanted to assess the effect of data selection on a problem where a non-linear deformation had been applied to  the data. 
Next we sampled on the non-linear deformation momenta, affine transformation parameters, permutation vector \emph{and} the data selection fidelity parameters, test c). The 8 chains converged to permutation vectors with between 2 and 9 incorrect matches. It was evident that the points with incorrect identified matches had reduced fidelity MAP estimators hence their contribution to the likelihood minimal, supplementary figure \ref{suppfig:deftest}a). \edit{The median cell to match distance was equal to 0.0943, table \ref{tab:defstats} and the identification of the correct permutation improved compared to when data selection was not included.} The high failure rate when we did not include data selection in test a) was suggestive of a rough, difficult to explore state space, this problem was significantly ameliorated by the inclusion of the fidelity parameters, resulting in improved performance and identification of cell matching. Overall this suggests that the inclusion of data selection could facilitate better mixing of chains and thus improve success in identification of the point matching.

As only a subsection of points were explicitly deformed in this test problem, we wanted to finally test whether the data selection could facilitate the matching of the un-deformed points when non-linear deformation was not included within our model, test d). We found the overall spatial matching of the un-deformed points to be greatly improved, with a  median cell to match distance, $\tilde{d_u}$, equal to 0.0342 (and $\tilde{d}=1.26$), table \ref{tab:defstats}. To visualise the matching we re-plotted the permutation heatmaps and ordered them according to the MAP estimates of the fidelity parameters, figure \ref{suppfig:deftest}a). All cells that were explicitly deformed had reduced contributions to the likelihood. Importantly, this shows that we are able to match the un-deformed region sufficiently well through the implementation of data selection. 

%To further investigate the effect of the fidelity parameters we compared the norm of the applied momenta for each cell with the MAP estimates of the fidelity parameters when we included sampling on the deformation and without, figure \ref{suppfig:deftest}b). When a non-linear deformation was included within the model, there was little correlation between applied momentum and fidelity (average Spearman's rank coefficient $\bar{\rho}=-0.182$). However, when non-linear deformation was not included within the model, the fidelity was correlated with momentum ($\bar{\rho}=-0.916$). This comparison suggests that the fidelity parameters tune out cells whose match cannot be described by the current model in a manner proportional to the level of model discrepancy and otherwise give a read-out on the relative error of the matched points. %%i think we should just get rid of this analysis , it doesnt really help, we know this is what the fidelity params are doing anyway 

These results are especially encouraging as the computational time is significantly reduced when we do not include non-linear deformation. %Additionally, the run-time does not scale significantly with $n$ when we sample only on the fidelity parameters (along with the affine parameters and permutation vector). 
We demonstrate that when a subset of points are subject to a complex, computationally demanding transformation, the fidelity parameters are able to account for these points and reduce their contribution to the overall matching, facilitating the accurate matching of the remaining points. In situations where the entire set of cells are subject to a complex transformation (e.g. non-linear deformation), then the fidelity parameter can encourage better mixing of the chains, thus improving the likelihood of finding a correct matching of points. 



%movie to fixed 


%rewrite from here on
%We identified distinct embryo and cell matching in 3 out of 4 of the embryos, table~\ref{tab:realtofixed}. We identified that embryos 1, 2, and 4 matched with embryos A, B, and C respectively, figure~\ref{fig:movietofixed} a-c). All 8 chains converged to the same permutation vector for each of these tests. 

% \begin{figure}[htpb]
%     \centering
%     \includegraphics{movietofixed.pdf}
%     \caption{}
%     \label{fig:movietofixed}
% \end{figure}

%We re-ordered the permutation heatmaps first according to the fidelity values at the MAP, and then by the probability of matching in $Y^2$, to obtain an approximately diagonal permutation probability heatmap, as in section~\ref{sec:fixedtofixed}, supplementary figures~\ref{suppfig:movietofixed}a) and~\ref{suppfig:movietofixed2}. Looking more closely at the MAP estimates of $\gamma$ we noticed that there were two matches with reduced fidelity means, supplementary figure~\ref{suppfig:movietofixed}a). These cells corresponded to cells 5 and 19 in $Y^1$ and cells 14 and 31 in $Y^2$, figure~\ref{suppfig:movietofixed}. Interestingly, these four cells appear in the extremes of the z axis (cells 5 and 31) and deep within the ICM (cells 14 and 19). Due to the embryo size, attenuation of confocal signal is expected along the z axis, making the upper z regions of images especially difficult to segment accurately. Additionally cell segmentation in denser regions of the ICM is more difficult leading to a higher risk of cell segmentation errors. From these observations and inference from the fidelity parameters we could go back to the original confocal images and re-assess the cell segmentation in these regions and check for cells that were not segmented correctly due to the attenuation of the nuclear signal. 

%However, for the matching of embryo 3 with embryo D, only 4 out of 8 chains converged to the same permutation vector, and the resulting cell to match distance significantly larger than the other three tests, figure~\ref{fig:movietofixed}d) and table~\ref{tab:realtofixed}. This reduction in matching accuracy may arise from inaccuracies during nuclear segmentation or potential deformation during fixation. We therefore re-ran the matching for embryo 3 and embryo D including inference of a geodesic flow for $N=2\times10^7$ tempered iterations and $N=10^6$ iterations at $T=1$. We identified 3/8 chains that reduced $\tilde{d}$, the minimum of which was equal to 0.122 suggesting a good matching of the points figure~\ref{fig:movietofixed}e). The identified fidelity parameters were also increased with only 7 cells with $\gamma_i<0.4$ as opposed to 22 cells when deformation was not included. \jf{I had a look at the permutation vectors for with and without deformation - they were different, but this is probably because there were lots of reduced fidelity means when we didnt include deformation. (Increase in number of points with higher fidelity when we DID include deformation} 

%movie to fixed stuff



\slc{We're so close here, but I think this last test below misses the point slightly. We've already made our points about median and RMSE changes with/without data selection. What we want to show here is that we end up with different MLMs if we do not do data selection (if indeed that is the case). We should also emphasise that only through data selection have we been able to match the embryos in a robust manner in the first place. We should report the average number of differences in the MLMs between the data selection and non data selection experiments. This bit can be kept extremely brief. Let me know if you'd like to discuss. If there aren't any "errors" then we should just drop it!}

To further assess the effect of data selection within these real tests, we then performed the cell matching for each of the identified embryo matches, without data selection. As we expected, we saw that the identified matching worked to minimise the overall RMSE distance and as a result the median cell to match distances increased, see table~\ref{tab:movienofid}. 

\begin{table}[htbp]
\centering
\begin{tabular}{c|c|c|}
\cline{2-3}
                                    & \textbf{Median} & \textbf{RMSE} \\ \hline
\multicolumn{1}{|c|}{\textbf{em1A}} & 1.118           & 0.970         \\ \hline
\multicolumn{1}{|c|}{\textbf{em2B}} & 0.240           & 0.137         \\ \hline
\multicolumn{1}{|c|}{\textbf{em3D}} & 1.029           & 0.785         \\ \hline
\multicolumn{1}{|c|}{\textbf{em4C}} & 0.424           & 0.233         \\ \hline
\end{tabular}
\caption{Median and RMSE cell to match distances for each embryo combination. Values given corresponding to the chain with the lowest negative log of the posterior distribution.}
\label{tab:movienofid}
\end{table}

Embryo 2 and embryo 4 were still well matched, with only a small increase in median cell to match distance and identification of a single unique MLM. However, embryo 1 displayed convergence to three different unique MLMs when data selection was not included, therefore reducing our confidence in the identified matching. This highlights our need to include the data selection framework to facilitate matching of the cells between potentially noisy data sets. Further to this, the inclusion of data selection facilitates further inference and interpretation on the confidence of the matches presented within the MLM. 

